A Unified Masked Autoencoder with Patchified Skeletons for Motion Synthesis

The synthesis of human motion has traditionally been addressed through task-dependent models that focus on specific challenges, such as predicting future motions or filling in intermediate poses conditioned on known key-poses. In this paper, we present a novel task-independent model called UNIMASK-M, which can effectively address these challenges using a unified architecture. Our model obtains comparable or better performance than the state-of-the-art in each field. Inspired by Vision Transformers (ViTs), our UNIMASK-M model decomposes a human pose into body parts to leverage the spatio-temporal relationships existing in human motion. Moreover, we reformulate various pose-conditioned motion synthesis tasks as a reconstruction problem with different masking patterns given as input. By explicitly informing our model about the masked joints, our UNIMASK-M becomes more robust to occlusions. Experimental results show that our model successfully forecasts human motion on the Human3.6M dataset. Moreover, it achieves state-of-the-art results in motion inbetweening on the LaFAN1 dataset, particularly in long transition periods. More information can be found on the project website https://evm7.github.io/UNIMASKM-page/

==> tables/ablation_lafan1.tex <==
\begin{table*}[]
\centering
\resizebox{0.65\textwidth}{!}{%
\begin{tabular}{@{}lccccccccc@{}}
  & \multicolumn{3}{c}{\textbf{L2Q $\downarrow$}}              & \multicolumn{3}{c}{\textbf{L2P $\downarrow$}}              & \multicolumn{3}{c}{\textbf{NPSS $\downarrow$}}                   \\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-10}
Num Transition Frames & \textbf{5}    & \textbf{15}   & \textbf{30}   & \textbf{5}    & \textbf{15}   & \textbf{30}   & \textbf{5}      & \textbf{15}     & \textbf{30}     \\ \midrule
w/o PD                                                           & 0.13                           & 0.34          & 0.59          & 0.15        & 0.50           & 1.03           & 0.0015          & 0.0227          & 0.1263          \\ 
w/o PA & 0.13                & 0.34                & 0.60                & 0.15                & 0.51                & 1.05                & 0.0015               & 0.0228               & 0.1271               \\
\midrule
w/ DCT                                                             & 0.17                           & 0.42          & 0.68          & 0.23        & 0.75           & 1.33           & 0.0019          & 0.0283          & 0.1503          \\
w/ TempMLP & \textbf{0.12} & 0.34 & 0.60 & \textbf{0.14} & 0.49 & 1.04 & \textbf{0.0014}          & 0.0226          & 0.1280           \\ \midrule
w/o $emb_{kin}$                                                & 0.13                           & 0.33          & 0.58          & 0.15        & 0.48           & 0.98           & \textbf{0.0014}          & 0.0221          & 0.1216          \\
w/ Attn Mask                                                    & 0.13                           & 0.34          & 0.59          & 0.15        & 0.49           & 1.02           & 0.0015          & 0.0226          & 0.1243          \\ \midrule
w/o encoder & \textbf{0.12} & \textbf{0.32} & 0.58 &\textbf{ 0.14} & 0.47 & 0.99 & \textbf{0.0014} & 0.0218 & 0.1248 \\
w/o decoder                                                        & 0.13                           & 0.34          & 0.60          & 0.16        & 0.51           & 1.05           & 0.0015          & 0.0228          & 0.1282          \\
MASK-M Light                                                        & 0.12                           & 0.33          & 0.59          & \textbf{0.14}        & 0.48           & 1.00           & \textbf{0.0014}          & 0.0022          & 0.1248          \\ \midrule
\textbf{MASK-M} & \multicolumn{1}{l}{{\textbf{0.12}}} & \textbf{0.32} & \textbf{0.57} & \textbf{0.14}  & \textbf{0.46}  & \textbf{0.97}  & \textbf{0.0014} & \textbf{0.0216} & \textbf{0.1204} \\ \hline
\end{tabular}%
}
\caption{Performance of our MASK-M under different configurations in the inbetweening task and the LaFan1 dataset \shortcite{lafan1dataset}. }
\label{tab:lafan1_ablation}
\end{table*}

==> tables/ablation_lafan1_short.tex <==
\begin{table}[]
\centering
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{@{}lccccccccc@{}}
  & \multicolumn{3}{c}{\textbf{L2Q $\downarrow$}}              & \multicolumn{3}{c}{\textbf{L2P $\downarrow$}}              & \multicolumn{3}{c}{\textbf{NPSS /1000 $\downarrow$}}                   \\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-10}
Num Frames & \textbf{5}    & \textbf{15}   & \textbf{30}   & \textbf{5}    & \textbf{15}   & \textbf{30}   & \textbf{5}      & \textbf{15}     & \textbf{30}     \\ \midrule
w/o PD                                                           & 0.13                           & 0.34          & 0.59          & 0.15        & 0.50           & 1.03           & 1.5          & 22.7          & 126.3          \\ 
w/o PA & 0.13                & 0.34                & 0.60                & 0.15                & 0.51                & 1.05                & 1.5               & 22.8               & 127.1               \\
\midrule
w/ DCT                                                             & 0.17                           & 0.42          & 0.68          & 0.23        & 0.75           & 1.33           & 1.9          & 28.3          & 150.3          \\
w/ TempMLP & \textbf{0.12} & 0.34 & 0.60 & \textbf{0.14} & 0.49 & 1.04 & \textbf{1.4}          & 22.6          & 128.0           \\ \midrule
w/o $emb_{kin}$                                                & 0.13                           & 0.33          & 0.58          & 0.15        & 0.48           & 0.98           & \textbf{1.4}          & 22.1          & 121.6          \\
w/ Attn Mask                                                    & 0.13                           & 0.34          & 0.59          & 0.15        & 0.49           & 1.02           & 1.5          & 22.6          & 124.3          \\ \midrule
w/o encoder & \textbf{0.12} & \textbf{0.32} & 0.58 &\textbf{ 0.14} & 0.47 & 0.99 & \textbf{1.4} & 21.8 & 124.8 \\
w/o decoder                                                        & 0.13                           & 0.34          & 0.60          & 0.16        & 0.51           & 1.05           & 1.5          & 22.8          & 128.2          \\
UNIMASK-M Light                                                        & 0.12                           & 0.33          & 0.59          & \textbf{0.14}        & 0.48           & 1.00           & \textbf{1.4}          & 2.2          & 124.8          \\ \midrule
\textbf{UNIMASK-M} & \multicolumn{1}{l}{{\textbf{0.12}}} & \textbf{0.32} & \textbf{0.57} & \textbf{0.14}  & \textbf{0.46}  & \textbf{0.97}  & \textbf{1.4} & \textbf{21.6} & \textbf{120.4} \\ \hline
\end{tabular}%
}
\caption{Performance of UNIMASK-M under different configurations in the inbetweening task for the LaFAN1 dataset.}
\label{tab:lafan1_ablation}
\end{table}

==> tables/comparison_synthesis.tex <==
\begin{table*}[]
\centering
\resizebox{0.72\textwidth}{!}{%
\begin{tabular}{@{}lcccccccccccc@{}}
\textbf{}                  & \multicolumn{6}{c}{\textbf{FORECASTING (MPJPE) $\downarrow$}}                                                                            & \multicolumn{6}{c}{\textbf{COMPLETION (MPJPE) $\downarrow$}}                                                      \\ \midrule
\textbf{Mask Probability} & \textbf{80}   & \textbf{160}  & \textbf{320}  & \textbf{400}  & \textbf{560}  & \multicolumn{1}{c|}{\textbf{1000}}  & \textbf{80}  & \textbf{160}  & \textbf{320}  & \textbf{400}  & \textbf{560}  & \textbf{1000} \\ \midrule
%Baseline          & 23,8          & 44,4          & 76,1          & 88,2          & 107,4         & \multicolumn{1}{c|}{136,6}          & 15,9         & 26,1          & 37,3          & 40,4          & 45,2          & 72,4          \\ \midrule
$1$     & \textbf{11.9}          & 25.1          & 50.7          & 61.6          & \textbf{79.6} & \multicolumn{1}{c|}{\textbf{112.1}} & 13.0                 & 23.7                 & 41.2                 & 47.5                 & 56.9                 & 82.2           \\
$0.9$     & \textbf{11.9}                              & 26.0          & 53.3          & 64.9          & 84.0         & \multicolumn{1}{c|}{117.5}              & \textbf{8,4} & \textbf{14.2} & \textbf{22.4} & \textbf{25.1} & \textbf{29.3} & 52.0          \\
$0.85 \rightarrow 1$        & \textbf{11.9} & \textbf{24.6} & \textbf{49.9} & \textbf{61.2} & 80.2          & \multicolumn{1}{c|}{115.7}                               & 8.5          & 14.7          & 22.9          & 25.7          & 29.9          & \textbf{51.9} \\ \bottomrule
\end{tabular}%
}
\caption{Performance comparison of MASK-M on Human3.6M dataset under different training masking strategies. Training on forecasting requires the whole future mask (mask probability of 1), while training on motion completion uses random patch masking (mask probability of 0.9). To enhance performance in both tasks, we use curricular learning that decreases the masking probability in training (from 0.85 to 1). We show that curricular learning finds optimal balance between both tasks.}
\label{tab:curricular learning}
\end{table*}

==> tables/computational_resources.tex <==
\begin{table}[]
\centering
\resizebox{0.40\textwidth}{!}{%
    \begin{tabular}{lcc}
    \textbf{Model} & \textbf{Parameters (M)}  & \textbf{Inference Time (ms)} \\ \midrule
    SiMLPe \shortcite{SIMPLE} & 0.14 & $7.86 \pm 0.05$\\
    STDGCN \shortcite{ST-DGCN} & 1.74 & $5.13  \pm 0.12$\\ \midrule
    U-CVAE \shortcite{UnifiedCVAE} & 8.50 & $9.30  \pm 0.44$\\
    MDM \shortcite{MDM} & 17.42 & $1683.50  \pm 50.31$\\ \midrule
    MASK-M (joints) & 2.42 & $3.98  \pm 0.05$ \\
    MASK-M (proposed) & 1.86 & $3.33  \pm 0.05$ \\
    \end{tabular}
}
\caption{Model size and average run time per 10000 runs.}
\label{tab:computationalresources}
\end{table}



==> tables/human36m_completion.tex <==
\begin{table}
\centering
\resizebox{0.36\textwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
milliseconds (ms) & \textbf{80}   & \textbf{160}        & \textbf{320}        & \textbf{400}        & \textbf{560}        & \textbf{1000}  \\ \midrule
Interpolation  & 15.9 & 26.1  & 37.3  & 40.4 & 45.2 & 72.4 \\ \midrule
CrossViT & 8.8.& 16.6 & 26.9& 30.0 & 34.3 & 56.4 \\
MASK-M (Ours) & \textbf{8.4} & \textbf{14.2} & \textbf{22.4} & \textbf{25.1} & \textbf{29.3} & \textbf{52.0}  \\  \bottomrule
\end{tabular}%
}
\caption{Quantitative comparison of MPJPE error in 3D human motion completion for Human3.6M dataset when 90\% of future joints are masked.}
\label{tab:quantitative_completion}
\end{table}

==> tables/lafan1_extend.tex <==
\begin{table}[]
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
  & \multicolumn{2}{c}{\textbf{L2Q $\downarrow$}}              & \multicolumn{2}{c}{\textbf{L2P $\downarrow$}}              & \multicolumn{2}{c}{\textbf{NPSS $\downarrow$}}                   \\ \cmidrule(lr){2-3}  \cmidrule(lr){4-5} \cmidrule(lr){6-7}
Transition Frames & \textbf{50}    & \textbf{70}  & \textbf{50}    & \textbf{70} & \textbf{50}    & \textbf{70}      \\ \midrule
$\Delta$-Interpolation   & 0.865                & 1.205                & 1.278                & 1.911                & 0.4042               & 1.018         \\
MASK-M    &\textbf{0.832}       & \textbf{1.16}        & \textbf{1.203}       & \textbf{1.796}       & \textbf{0.3716}      & \textbf{0.9532}      \\  \bottomrule
\end{tabular}%
}
\caption{Quantitative evaluation of human motion inbetweening on LAFAN1 dataset. Lower score is better.}
\label{tab:lafan1_extend}
\end{table}

==> tables/lafan1_quantitative.tex <==
\begin{table*}[]
\centering
\resizebox{0.80\textwidth}{!}{%
\begin{tabular}{@{}lccccccccc@{}}
  & \multicolumn{3}{c}{\textbf{L2Q $\downarrow$}}              & \multicolumn{3}{c}{\textbf{L2P $\downarrow$}}              & \multicolumn{3}{c}{\textbf{NPSS $\downarrow$}}                   \\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-10}
Transition Frames & \textbf{5}    & \textbf{15}   & \textbf{30}   & \textbf{5}    & \textbf{15}   & \textbf{30}   & \textbf{5}      & \textbf{15}     & \textbf{30}     \\ \midrule
Zero velocity         & 0.56 & 1.10 & 1.51 & 1.52 & 3.69 & 6.60 & 0.0053 & 0.0522 & 0.2318 \\
SLERP Interpolation   & 0.22 & 0.62 & 0.98 & 0.37 & 1.25 & 2.32 & 0.0023 & 0.0391 & 0.2013 \\ \midrule
TG$_{rec}$ \cite{lafan1dataset}                & 0.21 & 0.48 & 0.83 & 0.32 & 0.85 & 1.82 & 0.0025 & 0.0304 & 0.1608 \\
TG$_{complete}$  \cite{lafan1dataset}           & 0.17 & 0.42 & 0.69 & 0.23 & 0.65 & 1.28 & 0.0020 & 0.0258 & 0.1328 \\
SSMCT$_{local}$  \cite{TRANSFORMER_MIB1}          & 0.17 & 0.44 & 0.71 & 0.23 & 0.74 & 1.37 & 0.0019 & 0.0291 & 0.1430 \\
SSMCT$_{global}$  \cite{TRANSFORMER_MIB1}          & 0.14 & 0.36 & 0.61 & 0.22 & 0.56 & 1.10 & 0.0016 & 0.0234 & 0.1222 \\
$\Delta$-Interpolation  \cite{DELTA_INTERP}  & \textbf{0.11} & \textbf{0.32} & \textbf{0.57} & \textbf{0.13} & {\ul 0.47}    & {\ul 1.00}    & \textbf{0.0014} & {\ul 0.0217}    & {\ul 0.1215}    \\
%Tween Transformer     & 0.16 & 0.39 & 0.65 & 0.21 & 0.59 & 1.21 & 0.0019 & 0.0261 & 0.1358 \\
MASK-M (Ours)    & {\ul 0.12}    & \textbf{0.32} & \textbf{0.57} & {\ul 0.14}    & \textbf{0.46} & \textbf{0.97} & \textbf{0.0014} & \textbf{0.0216} & \textbf{0.1204} \\ \bottomrule
\end{tabular}%
}
\caption{Quantitative evaluation of human motion inbetweening on LAFAN1 dataset. Lower score is better.}
\label{tab:lafan1_quantitative}
\end{table*}

==> tables/patch_granularity_MF_MR.tex <==
\begin{figure}
\centering
\includegraphics[width=0.48\textwidth]{pics/PG_small.png}
\vspace{-0.7cm}
%\caption{\textbf{Different patch granularity strategies in Human3.6M skeleton.} }
\label{fig:patch_granularity}
\end{figure}
\begin{figure}[]
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{lcccccc}
 %\toprule
\textbf{Strategy} & \textbf{80} & \textbf{160} & \textbf{320} & \textbf{400} & \textbf{560} & \textbf{1000} \\  \midrule
S1 (joints) & 12.44 & 25.93 & 51.52 & 62.59 & 81.02 & 114.06 \\
S2 (body, w/o PD) & 12.38 & 25.92 & 51.57 & 62.62 & 80.60 &  {113.05} \\
\textbf{S3 (Proposed)} & 11.85 & 25.11 &  {50.69} &  {61.57} & \textbf{79.58 }& \textbf{112.10} \\
S4 (version 4)& \textbf{11.53} & \textbf{24.78 }& \textbf{50.24} &\textbf{ 61.38} &  {79.86} & 113.38 \\
S5 (version 5) &  {11.71} &  {24.93} & 50.58 & 61.78 & 80.54 & 113.31 \\ 
\end{tabular}
}
\vspace{0.05cm}
\caption{\textbf{MASK-M under different patch granularity.} MPJPE millimetre error of the motion forecasting task.}
\vspace{-4mm}
\label{tab:patch_granularity}
\end{figure}


